Single RGB-D Camera Teleoperation for General Robotic Manipulation

We propose a teleoperation system that uses a single RGB-D camera as the human motion capture device. Our system can perform general manipulation tasks such as cloth folding, hammering and 3mm clearance peg in hole. We propose the use of non-Cartesian oblique coordinate frame, dynamic motion scaling and reposition of operator frames to increase the flexibility of our teleoperation system. We hypothesize that lowering the barrier of entry to teleoperation will allow for wider deployment of supervised autonomy system, which will in turn generates realistic datasets that unlock the potential of machine learning for robotic manipulation. Demo of our systems are available online https://sites.google.com/view/manipulation-teleop-with-rgbd

==> table/teaser.tex <==
\begin{figure*}[!h]
\setlength{\tabcolsep}{1pt}
\begin{tabular}{cccc}
  \includegraphics[width=0.22\linewidth]{fig/tasks/pick_and_place.pdf} &   \includegraphics[width=0.22\linewidth]{fig/tasks/peg_in_hole.pdf} & \includegraphics[width=0.22\linewidth]{fig/tasks/hammer.pdf} &   \includegraphics[width=0.22\linewidth]{fig/tasks/cutting.pdf} \\
(a) Pick and Place & (b) Peg in Hole & (c) Hammering & (d) Cutting Fruit \\[6pt]
  \includegraphics[width=0.22\linewidth]{fig/tasks/cloth.pdf} &   \includegraphics[width=0.22\linewidth]{fig/tasks/drawer.pdf} & \includegraphics[width=0.22\linewidth]{fig/tasks/unknot.pdf} &   \includegraphics[width=0.22\linewidth]{fig/tasks/dual_arm.pdf} \\
(e) Folding Cloth & (f) Object Storage in Drawer & (g) Cord Untangling & (h) Moving Large Container\\[6pt]
\end{tabular}
\caption{We propose a teleoperation system which uses a single RGB-D camera to capture human motion. The human operator does not have access to any form of tactile feedback. Tasks (a)-(g) are evaluated on a real robot arm. Dual arm task (h) is performed in simulation. \vspace{-4mm}}
\label{fig:teaser}
\end{figure*}
